The Drinfeld associator of gl(1|1)

We determine explicitly a rational even Drinfeld associator Q in a completion of the universal enveloping algebra of the Lie superalgebra gl(1|1)^3. More generally, we define a new algebra of trivalent diagrams that has a unique even horizontal group-like Drinfeld associator P. The associator P is mapped to Q by a weight system. As a result of independent interest, we show how O. Viro's generalization Delta^1 of the multi-variable Alexander polynomial can be obtained from the universal Vassiliev invariant of trivalent graphs. We determine P by using the invariant Delta^1(T) of a planar tetrahedron T.

==> cij.tex <==
%auto-ignore
\begin{picture}(0,0)%
\includegraphics{cij.eps}%
\end{picture}%
\setlength{\unitlength}{4144sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(32,555)(251,164)
\put(251,164){\makebox(0,0)[lb]{\smash{\SetFigFont{8}{9.6}{\familydefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$1$}%
}}}
\put(251,614){\makebox(0,0)[lb]{\smash{\SetFigFont{8}{9.6}{\familydefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$1$}%
}}}
\end{picture}


==> rel2.tex <==
%auto-ignore
\begin{picture}(0,0)%
\includegraphics{rel2.eps}%
\end{picture}%
\setlength{\unitlength}{3947sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(838,361)(182,50)
\put(541,178){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{\familydefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$=$}%
}}}
\end{picture}

